The ubiquity of conservative translations

We study the notion of conservative translation between logics introduced by Feitosa and D'Ottaviano. We show that classical propositional logic (CPC) is universal in the sense that every finitary consequence relation over a countable set of formulas can be conservatively translated into CPC. The translation is computable if the consequence relation is decidable. More generally, we show that one can take instead of CPC a broad class of logics (extensions of a certain fragment of full Lambek calculus FL) including most nonclassical logics studied in the literature, hence in a sense, (almost) any two reasonable deductive systems can be conservatively translated into each other. We also provide some counterexamples, in particular the paraconsistent logic LP is not universal.

==> defs.tex <==
\ifx\mydefs\undefined\else\endinput\fi
\let\mydefs\relax

%%%%% GENERAL STUFF

\linespread{1.1}
\allowdisplaybreaks[2]

\ifx\loadcyr\undefined\else
\input cyracc.def
\makeatletter
\font\elvcyr=wncyr10 at 1\@ptsize pt
\font\elvcyb=wncyb10 at 1\@ptsize pt
\font\elvcyi=wncyi10 at 1\@ptsize pt
\makeatother
\def\cyr{\elvcyr\cyracc}
\def\cyb{\elvcyb\cyracc}
\def\cyi{\elvcyi\cyracc}
\fi

%obsolete
%-\newcounter{Case}
%-\def\Cases{\setcounter{Case}0}
%-\def\case{\par\pagebreak[2]\medskip\noindent\refstepcounter{Case}%
%-   \textbf{Case \theCase:}\bme\ignorespaces}

\hyphenation{ir-re-flex-ive}


%%%%% SYMBOLS

%%% auxiliary macros

\let\M\mathit
%-\def\defsym#1#2{\def#1{\ensuremath{\M{#2}}}}
\def\gobble#1{}
\def\fixsup#1#2{{#1\let\dp\gobble\mathstrut}^#2_}
\let\mr\mathrel
%-\def\sch#1{-$\M{#1}$}
\let\me\enskip
\def\bme{\hskip.75em\relax}


%%% general logic

%%\def\nee{\mathord\sim}
%-\let\nee\neg
%\def\et{\mathbin\&}
\let\et\land
\let\eq\leftrightarrow
\let\EQ\Leftrightarrow
\def\nequiv{\not\equiv}
\def\iff{\quad\text{iff}\quad}
\let\LOR\bigvee%\limits ?
\let\ET\bigwedge%\limits ?
\let\TO\Rightarrow
\def\?{\mathbin?}
\let\ot\leftarrow
\let\Lto\supset
\let\Leq\equiv
\let\model\vDash
\let\nmodel\nvDash

\newbox\circlebox
\setbox\circlebox\hbox{$\bigcirc$}
\def\circled#1{%
  \setbox0\hbox to\wd\circlebox{\hss$#1$\hss}\wd0=0pt
  \box0\copy\circlebox}
\def\cand{\mathbin{\circled\land}}
\def\cor{\mathbin{\circled\lor}}
\def\ccir{\mathbin{\circled\circ}}
\def\cneg{\circled\neg}


%%% greek

\let\fii\varphi
\let\tet\vartheta
\let\ep\varepsilon
\let\kap\varkappa
\let\roo\varrho
\def\greek#1{$\expandafter\greeknum\csname c@#1\endcsname$}
\makeatletter
\def\greeknum#1{\ifcase#1\or\alpha\or\beta\or\gamma\or\delta\or\ep
      \or\digamma\or\zeta\or\eta\or\tet\or\iota\else\@ctrerr\fi}
\makeatother


%%% sets, functions, sequences

\def\p#1{\langle#1\rangle}
\def\vp#1{[#1]}
\def\lh#1{\lvert#1\rvert}
\let\abs\lh
\let\cat\smallfrown
%\def\ccat{\mathbin\frown}%\smallsmile
%\let\vec\overline
\let\lvec\overrightarrow
\let\bez\smallsetminus
\let\sdif\vartriangle
\let\sset\subseteq
\let\nsset\nsubseteq
\let\Sset\supseteq
\let\nSset\nsupseteq
\let\onto\twoheadrightarrow
\let\otno\twoheadleftarrow
\let\embed\hookrightarrow%\rightarrowtail
\def\cupd{\mathbin{\dot\cup}}
%\def\bigcupd{\mathop{\overset{\text{\large.}}{\bigcup}}} why was that?
\def\bigcupd{\mathop{\dot\bigcup}}
%\let\bigcupd\sum
\def\pw#1{\mathcal P(#1)}
\let\nul\varnothing
\def\res{\mathbin\restriction}
\let\bd\partial
\def\two{\mathbf2}
\def\iim{^{-1\twoprimes}}
\def\img{^{%\mkern1mu hmmmm
\,\twoprimes}}
% 0.2\fontdimen etc. = 18/5 mu
\def\twoprimes{\raise.2\fontdimen6\scriptfont2\hbox{$\scriptstyle\prime\prime$}}
%full-featured version:
%\def\iim{^{-1\twoprimes}}
%\def\img{^{\mkern1mu\twoprimes}}
%\def\twoprimes{\mathchoice{}{}%
%   {\ttwoprimes\scriptfont\scriptstyle}%
%   {\ttwoprimes\scriptscriptfont\scriptscriptstyle}}
%\def\ttwoprimes#1#2{\raise .2\fontdimen 6 #12
%   \hbox{\mathsurround 0pt$#2\prime\prime$}}
%

%retraction pairs:
\newcommand\rpair[3][3em]{\mathrel{%
   \begin{matrix}%
     \strut\smash{\xrightonto{\hbox to#1{\hss$#2$\hss}}}\\[-1.7ex]%
     \strut\smash{\xleftembed[\hbox to#1{\hss$#3$\hss}]{}}%
   \end{matrix}}}
\makeatletter
%after tex/latex/amsmath/amsmath.sty:
%%\newcommand{\xrightarrow}[2][]{\ext@arrow 0359\rightarrowfill@{#1}{#2}}
%%\newcommand{\xleftarrow}[2][]{\ext@arrow 3095\leftarrowfill@{#1}{#2}}
\newcommand\xrightonto[2][]{\ext@arrow 0359\rightontofill{#1}{#2}}
\newcommand\xleftembed[2][]{\ext@arrow 3095\leftembedfill{#1}{#2}}
%%\def\leftarrowfill@{\arrowfill@\leftarrow\relbar\relbar}
%%\def\rightarrowfill@{\arrowfill@\relbar\relbar\rightarrow}
\def\leftembedfill{\arrowfill@\leftarrow\relbar\hookleftnoarrow}
\def\rightontofill{\arrowfill@\relbar\relbar\onto}
%%\renewcommand{\hookleftarrow}{\DOTSB\leftarrow\joinrel\rhook}
\def\hookleftnoarrow{\DOTSB\relbar\joinrel\rhook}
\makeatother

%%% arithmetic

\def\code#1{\ulcorner#1\urcorner}
\let\num\overline
%\def\div#1#2{\lfloor\frac{#1}{#2}\rfloor}
\def\div{\genfrac\lfloor\rfloor{}{}}
\def\tdiv{\genfrac\lfloor\rfloor{}1}
\def\dive#1#2{\div{#1}{2^{#2}}}
\def\tdive#1#2{\lfloor#1/2^{#2}\rfloor}
\def\rem{\mathbin{\mathrm{rem}}}
\def\ljk{\genfrac(){}{}}
\def\mljk{\genfrac[]{}{}}
\def\tljk#1#2{(#1|#2)}
\def\tmljk#1#2{[#1|#2]}
\def\mbin{\genfrac[]{0pt}{}}
\def\fl#1{\lfloor#1\rfloor}
\def\Fl#1{\left\lfloor#1\right\rfloor}
\def\cl#1{\lceil#1\rceil}
\def\CL#1{\left\lceil#1\right\rceil}
\mathchardef\#="2023 % \mathbin\#
\def\varsm{\mathbin{\overline\#}}
\def\tr#1{\lVert#1\rVert}%\left\|...\right\| ?
\def\str#1{[\mkern-2.7mu[#1]\mkern-2.7mu]}% \mathbb[ doesn't work
\def\mtr#1{\{\mkern-6mu\{#1\}\mkern-6mu\}}
%\def\divi{\mathrel|}
\let\divi\mid
\let\leg\lesseqqgtr
\let\ass\leftarrow
\let\hash\looparrowright
\let\ale\precsim
\def\nale{\not\precsim}
\def\Tr{{\mathrm T}}
\def\mnr#1#2{[#1;#2]}
\def\mat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\dmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\rsuv{\M{RSUV}}
\def\bmd{\mathbin\%}
\def\dle{\mathrel{\dot\le}}
\def\tsum{\textstyle\sum}

%%% sequent calculus

%\let\seq\Longrightarrow
%\let\seq\longrightarrow
\let\seq\vdash
\def\lft#1{\hbox{$#1$-l}}
\def\rgt#1{\hbox{$#1$-r}}

\ifx\busspf\undefined\else
\usepackage{bussproofs}
\EnableBpAbbreviations
\def\fCenter{\mathstrut\seq}
\let\LL\LeftLabel
\let\RL\RightLabel
\fi

%%% modal stuff

\let\dia\Diamond
\def\diadot{\centerdot\dia}
\ifx\symlasy\undefined
  \let\origboxdot\boxdot
  \def\boxdot{\mathord\origboxdot}
  \def\centerdot#1{%
    % NB: straightforward centering of two boxes does not work in this
    % case, due to negative depth of some of the characters. Hence the
    % \mathop business.
    \setbox0\hbox{$\mathop{#1}$}\dimen0 \ht0
    \setbox0\hbox{$#1$}\advance\dimen0 -\ht0
    \setbox2\hbox to\wd0{\hss$\mathop{\cdot}$\hss}\wd2=0pt
    \lower\dimen0\box2\box0 }
\else
  % lasy font metric is wrong, PR latex/3838
  \def\boxdot{\centerdot\Box}
  \def\centerdot#1{%
     \setbox0\hbox{$#1$}%
     \raise0.206\ht0\hbox to\wd0{\hss$\cdot$\hss}%
     \kern-\wd0 \box0 }
\fi
\def\T{\mathsf T}
\def\adm{\mathrel{|\mkern-8.5mu\sim}}
\def\nadm{\mathrel{|\mkern-8.5mu\not\sim}}
%-\def\Adm{\mathrel{|\approx}}
\let\ad\vartriangleright
%\def\isu{\mathrel{<\llap{$\cdot$}}}
\let\isu\lessdot
\def\ru{\mathrel/}
\def\Ru{\Bigm/}
\let\sls|
\def\up{\mathord\uparrow}
\def\down{\mathord\downarrow}
\def\Up{{\setbox0\hbox{$\uparrow$}%
         \lower\dp0\hbox to\wd0{\hss\vrule width4pt height.4pt\hss}%
         \kern-\wd0\box0}}
\def\UP{{\setbox0\hbox{$\uparrow$}%
         \lower\dp0\hbox to\wd0{\hss\vrule width4pt height.4pt\hss}%
         \kern-\wd0\copy0\kern-\wd0\raise.35ex\box0}}
\def\Down{{\setbox0\hbox{$\downarrow$}%
         \raise\ht0\hbox to\wd0{\hss\vrule width4pt depth.4pt\hss}%
         \kern-\wd0\box0}}
\def\sgen{\mathrel{\mathord\subseteq\cdot\!}}
\let\for\Vdash
%-\def\For#1{\mathrel{\Vdash^{#1}\negmedspace}}
\let\nfor\nVdash


%%% rm operators

\DeclareMathOperator\dom{dom}
\DeclareMathOperator\rng{rng}
\DeclareMathOperator\bit{bit}
\DeclareMathOperator\card{card}
\DeclareMathOperator\Size{Size}
\DeclareMathOperator\id{id}
\DeclareMathOperator\Lh{lh}
\DeclareMathOperator\md{md}
\DeclareMathOperator\cls{cl}%\cl clashes
\let\Pr\relax
\DeclareMathOperator\Pr{Pr}%get rid of \displaylimits
\DeclareMathOperator\E{E}
\DeclareMathOperator\var{var}
\DeclareMathOperator\cont{cont}
\DeclareMathOperator\Cut{Cut}
\DeclareMathOperator\Log{Log}
\DeclareMathOperator\LogLog{LogLog}
\DeclareMathOperator\wit{Wit}
\DeclareMathOperator\Hard{Hard}
\DeclareMathOperator\eval{eval}
\DeclareMathOperator\Eval{Eval}
\DeclareMathOperator\Circ{Circ}
\DeclareMathOperator\Th{Th}
\DeclareMathOperator\Mod{Mod}
\DeclareMathOperator\Df{Def}
\DeclareMathOperator\Var{Var}
\DeclareMathOperator\Form{Form}
\DeclareMathOperator\BS{BS}
\DeclareMathOperator\prf{Prf}
\DeclareMathOperator\clq{Clique}
\DeclareMathOperator\clr{Colour}
\def\hard{\Hard_}
\def\avhd{\Hard^A_}
\DeclareMathOperator\Ext{Ext}
\DeclareMathOperator\NExt{NExt}
\DeclareMathOperator\su{s}
\DeclareMathOperator\Aut{Aut}
\DeclareMathOperator\Gal{Gal}
\DeclareMathOperator\sgn{sgn}
\DeclareMathOperator\Int{int}%\int clashes
\DeclareMathOperator\chull{C}
\DeclareMathOperator\rcl{rcl}
\DeclareMathOperator\acl{acl}
\DeclareMathOperator\Res{Res}
\DeclareMathOperator\Ind{Ind}
\DeclareMathOperator\dist{dist}
%redefine the ugly Re, Im:
\let\Re\relax
\let\Im\relax
\DeclareMathOperator\Re{Re}
\DeclareMathOperator\Im{Im}

%%% complexity classes

\let\cxt\mathrm
\def\np{\cxt{NP}}
\def\conp{\cxt{coNP}}
\def\pnp{\cxt{prNP}}
\def\rp{\cxt{RP}}
\def\corp{\cxt{coRP}}
\def\bpp{\cxt{BPP}}
\def\pbpp{\cxt{prBPP}}
\def\zpp{\cxt{ZPP}}
\def\ma{\cxt{MA}}
\def\pma{\cxt{prMA}}
\def\am{\cxt{AM}}
\def\coam{\cxt{coAM}}
\def\pam{\cxt{prAM}}
\def\app{\cxt{APP}}
\def\ptime{\cxt P}
\def\prp{\cxt{prP}}
\def\ph{\cxt{PH}}
\def\fp{\cxt{FP}}
\def\CAPP{\M{CAPP}}
\DeclareMathOperator\poly{poly}
\def\wpwit{\M{WPHPWIT}}
\def\mfpp{\cxt{MFRP}}
\def\frp{\cxt{FRP}}
\def\tfrp{\cxt{TFRP}}
\def\pptm{\M{PPTM}}
\def\tfzpp{\cxt{TFZPP}}
\def\ppa{\cxt{PPA}}
\def\ppad{\cxt{PPAD}}
\def\ppp{\cxt{PPP}}
\def\pwpp{\cxt{PWPP}}
\def\nc{\cxt{NC}}
\def\nci{\nc^1}
\def\nca{\nci_*}
\def\psp{\cxt{PSPACE}}
\def\tc{\cxt{TC}^0}
\def\Ac{\cxt{AC}^0}
\def\task#1{{\normalfont\textsc{#1}}}
\def\pig{\task{Pigeon}}
\def\wpig{\task{WeakPigeon}}
\def\lone{\task{Lonely}}
\def\fac{\task{Factoring}}
\def\ffac{\task{FullFac}}
\def\fsr{\task{FacRoot}}
\def\wfsr{\task{WeakFacRoot}}
\def\fsrm{\task{FacRootMul}}
\def\fsro{\task{FacRootOdd}}
\def\fsre{\task{FacRootEven}}
\def\sroot{\task{Root}}
\def\qrec{\task{QuadRec}}

%%% theories

\def\sig{\Sigma^b_}
\def\pii{\Pi^b_}
\def\delt{\Delta^b_}
\def\delz{\Delta_0}%^0
\def\Sig{\Sigma^B_}
\def\Pii{\Pi^B_}
\def\Delt{\Delta^B_}
\def\st{\expandafter\hat}
\def\io{\M{IOpen}}
\def\idz{I\Delta_0}
\def\bas{\M{BASIC}}
\def\pv{PV}
\def\tpv{PV_1}
\def\sss{S^1_2}
\def\ttt{T^0_2}
\def\tv{\M{TV}^0}
\def\vtc{\M{VTC}^0}
\def\vtcim{\vtc+\M{IMUL}}
\def\vnc{\M{\!VNC}^1}
\def\vnca{\M{\!VNC}^1_*}
%\def\vncba{\overline{\M{VNC}}\setbox0\hbox{$\textstyle{\M{C}}$}\setbox2\null\ht2=\ht0\dp2=\dp0\box2^1_*}
\def\vncba{\overline{\M{\!VNC}}{\def\mathpalette##1{##1{}}\vphantom{C}^1_*}}
\def\lvncba{L_{\overline{\M{\!VNC}}{\def\mathpalette##1{##1{}}\vphantom{\scriptstyle C}^1_*}}}
%-\def\sigc{\fixsup\Sigma c}
%-\def\piic{\fixsup\Pi c}
%-\def\delc{\fixsup\Delta c}
%-\def\lc{L_{\M{Cnt}}}
%-\def\cnt{\M{Cnt}_}
%-\def\cq{\mathbf C^}
%-\def\cth{C^1_2}
%-\def\Gcth{GC^1_2}
\def\BB{\M{BB}}
\def\bbs{\BB\sig1}
%-\def\php{\M{sPHP}}
\def\php{\M{PHP}}
\def\sphp{\M{sPHP}}
\def\iphp{\M{iPHP}}
\def\rphp{\M{rPHP}}
\def\mphp{\M{mPHP}}
%-\def\wphp{\M{sWPHP}}
\def\wphp{\M{WPHP}}
\def\swphp{\M{sWPHP}}
\def\iwphp{\M{iWPHP}}
\def\rwphp{\M{rWPHP}}
\def\mwphp{\M{mWPHP}}
\def\thard{\M{HARD}_}
\def\tavhd{\M{HARD}^A}%!!! _}
\def\bt{\tpv+\swphp(\pv)}
%\def\bts{T^1_2+\php(\fp^{\sig1})}
\def\bts{T^1_2+\swphp(\pv_2)}%\pv(\sig1))}
\def\btr{T^1_2+\rwphp(\pv_2)}%\pv(\sig1))}
\def\bta{\tpv(\alpha)+\swphp(\pv(\alpha))}
\def\fpsa{\pv_2(\alpha)}%\pv(\sig1(\alpha))}
\def\btsa{T^1_2(\alpha)+\swphp(\fpsa)}
\def\btra{T^1_2(\alpha)+\rwphp(\fpsa)}
%-\def\fpsl{\fp^{\sig1(\alpha)[\mathrm{wit},\log]}}
%-\def\wbts{S^1_2(\alpha)+\swphp(\fpsl)}
%-\def\wbtr{S^1_2(\alpha)+\rwphp(\fpsl)}
%\def\lhmin{\sch{LENGTH}\sch{MIN}}
%\def\lhmax{\sch{LENGTH}\sch{MAX}}
\def\lhmin{$\M{LMIN}$}
\def\lhmax{$\M{LMAX}$}
\def\lind{$\M{LIND}$}
\def\pind{$\M{PIND}$}
\def\ind{$\M{IND}$}
\def\comp{$\M{COMP}$}
\def\compb{$\overline{\M{COMP}}$}
\def\scv{$\M{SCV}$}
\def\scvb{$\overline{\M{SCV}}$}
\def\ac{$\M{AC}$}
\def\acr{$\M{CR}$}
\def\coun{\M{Count}}
\def\open{\M{Open}}
\def\la{\M{LA}}
\def\lap{\M{LAP}}
\def\vlap{\M{\forall LAP}}
\def\mlap{\M{\forall LAP^-}}
\def\ik{\M{IK}}
\def\ikm{\M{IK^-}}
\def\ikz{\M{IK}_0}
\def\PA{\M{PA}}
\def\rcf{\M{RCF}}
\def\grh{\M{GRH}}
\def\grhq{\M{GRH_q}}


%%% logics, proof systems

\let\lgc\mathbf
\let\ax\mathrm
\def\EF#1{#1\text-\M{EF}}
\def\SF#1{#1\text-\M{SF}}
\def\CF#1{#1\text-\M{CF}}
\def\Fr#1{#1\text-\M{F}}
\def\TL#1#2{#1{#2}^*}
\def\CPC{\lgc{CPC}}
\def\IPC{\lgc{IPC}}
\def\MTL{\lgc{MTL}}
\def\BL{\lgc{BL}}
\def\luk{\textbf{\textup\L}}
%should avoid:
 \def\gl{\M{GL}}
 \def\gla{\M{GLA}}
 \def\glal{\M{GLAL}}
 \def\agl{A_{GL}^\Box}
\def\cf#1#2{\alpha(#1,#2)}
\def\qcf#1#2{\alpha^\bullet(#1,#2)}
\def\I{{\bullet}}
\def\R{{\circ}}
\def\RI{*}
\let\F\sharp
%\let\sng\widehat
\def\sng#1{\lowercase{#1}^}
\def\mon{{\mathbf m}}
%-\def\K{K^\forall}
%-\def\HK{\M{HK}^\forall}
%-\def\GK{\M{GK}^\forall}
%\def\MLL{\M{MLL}}
\def\mlk{\M{MLK}}
\def\lk{\M{LK}}
\def\mclk{\M{MCLK}}
\def\G{G}
\def\stG{\hat G}
\def\WDP{\M{WDP}}
\def\CC{\M{CC}}
\def\RCC{\M{RCC}}
\def\NA{\M{NA}}
\def\siq{\Sigma^q_}
\def\piq{\Pi^q_}
\def\FL#1{\lgc{FL_{#1}}}

%%% structures

\def\N{\mathbb N}
\def\Q{\mathbb Q}
\def\Z{\mathbb Z}
\def\RR{\mathbb R}%\R clashes
\def\C{\mathbb C}
\def\qlog{\Q_{\Log}}
\def\zg{\fixsup\Z*}
\def\cg#1{C(#1)}
%\def\GF#1{\M{GF}(#1)}
\def\GF#1{\mathbb F_{#1}}
\let\stm\N
\def\ukiv{U_0(K4)}
\def\rn{\M{RN}}

%%% misc

%\def\ast{\mathord*}% redef.!
\mathcode`\*="0203
\let\ob\overline
\def\tria{{\vartriangle}}
\mathchardef\mhyphen="2D

%%%%% THEOREMS

\def\noproof{\leavevmode\unskip\bme\vadjust{}\nobreak\hfill$\qed$\par}
\let\qed\Box
\newenvironment{Pf}[1][]
  {\par\noindent\textit{Proof\optpar{#1}:}\bme\ignorespaces}
  {\noproof\pagebreak[2]\vskip\medskipamount\ignorespacesafterend}
%UWAGA: \medskip -> \vspace\medskipamount -> ... ->
%       ->  \vskip\medskipamount \vskip 0pt  a to nechci
\def\qedhere{\relax\ifmmode\eqno\qed\expandafter\aftergroup
                   \else\noproof\fi\noqed}
\def\noqed{\let\noproof\relax}

\theoremstyle{plain}
\ifx\shortthm\undefined
\newtheorem{Thm}{Theorem}[section]
\else
\newtheorem{Thm}{Theorem}
\fi
\newtheorem{Prop}[Thm]{Proposition}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Lem}[Thm]{Lemma}
\newtheorem{Fact}[Thm]{Fact}
\newtheorem{Obs}[Thm]{Observation}
\newtheorem{Conj}[Thm]{Conjecture}
\newtheorem{Que}[Thm]{Question}
\newtheorem{Prob}[Thm]{Problem}
\newtheorem{Ass}[Thm]{Assumption}
\newtheorem{Cl}{Claim}[Thm]
\def\theCl{\arabic{Cl}}
\def\qedCl{\Box\hbox{ (Claim \theCl)}}
\theorembodyfont\upshape
\newtheorem{Def}[Thm]{Definition}
\newtheorem{Rem}[Thm]{Remark}
\newtheorem{Exm}[Thm]{Example}
\newtheorem{Expl}[Thm]{Explanation}
\newenvironment{Pf*}{\let\qed\qedCl\Pf}\endPf
\def\theequation{\arabic{equation}}


%%%%% HACKS

% %%% references with automatic theorem names:

% % \begin{Lem}\thlabel{xyz}...
% %
% % \thref{xyz} -> "Lemma 5.7.7"
% % \ref{xyz}  -> "5.7.7"
% % \thnameref{xyz}-> "Lemma"
% % \thref{xyz,pqr,abc} -> "Lemma 5.7.7 and Theorems 2.1.5 and 6.6.4"
%
\usepackage[reftex]{theoremref}
% \makeatletter
%   %hook in \@thm to get the name
%   \let\origthm\@thm
%   \def\newthm#1#2{\thmlowercase{\def\currthmname{#2}}\origthm{#1}{#2}}
%   \def\amsnewthm#1#2#3{\thmlowercase{\def\currthmname{#3}}\origthm{#1}{#2}{#3}}
%   \@ifpackageloaded{amsthm}{\let\@thm\newamsthm}{\let\@thm\newthm}
% %  for lowercase names, replace next \def with
% %  \let\thmlowercase\lowercase
%   \def\thmlowercase#1{#1}
%   %hacked version of \label from the kernel
%   %put the theorem name in the useless slot for page number
%   \def\thlabel#1{\@bsphack
%     \protected@write\@auxout{}%
%            {\string\newlabel{#1}{{\@currentlabel}{\currthmname}}}%
%     \@esphack}
%   %\let\thnameref\pageref breaks badly when the ref is undefined
%   \def\thnameref#1{\expandafter\mysetref\csname r@#1\endcsname}
%   \def\mysetref#1{\ifx#1\relax?THM?\else\expandafter\@secondoftwo#1\fi}
% \makeatother
% \newif\ifrefcomma \newif\iffinalcomma \newcount\refnum
% \def\thref#1{\let\lastname\empty\let\refstack\empty\let\refhead\empty
%   \refcommafalse\finalcommafalse\dothref#1,,}
% \def\dothref#1,{\ifx,#1,\ifrefcomma\iffinalcomma,\fi\space and \fi
%     \refcommafalse\expandafter\flushref
%   \else\edef\thisname{\thnameref{#1}}\ifx\thisname\lastname
%       \let\do\relax\edef\refstack{\refstack\do{\refhead}}%
%     \else\flushref\let\lastname\thisname\fi
%     \def\refhead{#1}\expandafter\dothref\fi}
% \def\flushref{\ifx\lastname\empty\else
%     \ifrefcomma, \finalcommatrue\fi\refcommatrue
%     \lastname\ifx\refstack\empty\else s\fi\refnum 0
%     \let\do\onethref\refstack\ifcase\refnum\or\space and\else
%       \finalcommatrue, and\fi~$\ref{\refhead}$\let\refstack\empty\fi}
% \def\onethref#1{\ifnum\refnum>0,\fi\space$\ref{#1}$\advance\refnum 1 }
% %this is a hack to make reftex.el happy:
% %can use \th\label, \th\ref instead of \thlabel, \thref
% \def\th#1{\csname th\expandafter\gobble\string#1\endcsname}

%%% algorithms:
\newif\iflinenumbers
\linenumberstrue
\newenvironment{algo}[1][20em]{\catcode`\^^I=13 \obeylines\doalgo{#1}}{}
{\catcode`\^^I=13 \catcode`\^^M=13
\gdef\doalgo#1#2\end#{\hbox to\hsize{\hss \let^^I\qquad%
  \def\\^^M{\nobreak\hfil\break\vadjust{}\qquad}%
  \fboxsep1em \linenum0 %
  \fbox{\hsize#1\vbox{%
  \everypar{\advance\linenum1 %
      \hbox to1.2em{%
           \hss\iflinenumbers$\scriptstyle\the\linenum$\hskip.6em\fi}}%
  #2}}\hss}\end}}
\newcount\linenum
\def\comment#1{\emph{/* #1 */}}
\def\key{\relax\ifmmode\expandafter\mathbf\else\expandafter\textbf\fi}
%\def\key#1{{\bf#1}} breaks at the beginning of a line


%%% upshape parentheses:

\def\allowhyphens{\nobreak\hskip0pt\relax}
\def\hyph{\allowhyphens-\hskip0pt\relax}
\DeclareRobustCommand*\magiclparen{\ifmmode(\else\textup(\allowhyphens\fi}
\DeclareRobustCommand*\magicrparen{\ifmmode)\else\textup)\fi}
\let\lparen=(  \let\rparen=)
\def\magicparon{\catcode`\(\active\catcode`\)\active}
\def\magicparoff{\catcode`\(12 \catcode`\)12 }
%active parens break preview-latex.el:
\AtBeginDocument{\ifx\ifPreview\iftrue\else\magicparon\fi}
\magicparon
\let (=\magiclparen  \let )=\magicrparen

%%% labels etc.: here because it uses ( )
\def\theenumi{\roman{enumi}}
\ifx\enumup\undefined
  \def\labelenumi{(\textit\theenumi)}
\else
  \def\labelenumi{(\theenumi)}
\fi
\def\theenumii{\greek{enumii}}
\def\labelenumii{(\theenumii)}
\def\optpar#1{\ifx\relax#1\relax\else\/ (#1)\fi}
%\def\DT#1{(in $#1$)}
\def\DT#1{(in $#1$)\pretolerance-1\nobreak\hfil\penalty1000\hfilneg}
%(\hfil in a line forces zero badness, which essentially means that
%TeX would never make it into pass 2, and will choose to break the
%line badly after the \DT even if better solution exists with hyphenation.
%Hence the \pretolerance=-1. The alternative of using finite
%stretchability seems to do more harm than good.)
\magicparoff


%%% allow line breaks after commas, for use in longish \p{...}

\def\cmb{\mathcode`\,"8000 }
\mathchardef\comma=\mathcode`\,
{\catcode`\,=\active \gdef,{\comma\penalty\relpenalty}}


%%%%% FRONT MATTER

\providecommand\dedic{\thanks{Supported by
grant IAA100190902 of GA AV \v CR, Center of Excellence CE-ITI under the grant
P202/12/G061 of GA \v CR, and RVO: 67985840.}}
\author{Emil Je\v r\'abek\dedic\\[\medskipamount]
Institute of Mathematics of the Academy of Sciences\\
\small \v Zitn\'a 25,
115\:67 Praha 1,
Czech Republic,
email: \texttt{jerabek@math.cas.cz}
%URL: \texttt{http://math.cas.cz/\string~jerabek}
}

\endinput

